Can LLMs Outshine Conventional Recommenders? A Comparative Evaluation

In recent years, integrating large language models (LLMs) into recommender systems has created new opportunities for improving recommendation quality. However, a comprehensive benchmark is needed to thoroughly evaluate and compare the recommendation capabilities of LLMs with traditional recommender systems. In this paper, we introduce RecBench, which systematically investigates various item representation forms (including unique identifier, text, semantic embedding, and semantic identifier) and evaluates two primary recommendation tasks, i.e., click-through rate prediction (CTR) and sequential recommendation (SeqRec). Our extensive experiments cover up to 17 large models and are conducted across five diverse datasets from fashion, news, video, books, and music domains. Our findings indicate that LLM-based recommenders outperform conventional recommenders, achieving up to a 5% AUC improvement in the CTR scenario and up to a 170% NDCG@10 improvement in the SeqRec scenario. However, these substantial performance gains come at the expense of significantly reduced inference efficiency, rendering the LLM-as-RS paradigm impractical for real-time recommendation environments. We aim for our findings to inspire future research, including recommendation-specific model acceleration methods. We will release our code, data, configurations, and platform to enable other researchers to reproduce and build upon our experimental results.

==> Assets/Tables/exp-zero-shot-pair.tex <==
\begin{table}[t]
\centering
% \renewcommand{\arraystretch}{1.2} 
% \setlength\tabcolsep{3pt}


\caption{LLM zero-shot performance in the pair-wise recommendation scenario. We display AUC metric in this table. Latency is the averaged inference time per sample.}\label{tab:zero-shot}

% \resizebox{\linewidth}{!}{
\begin{tabular}{llllllll}
\toprule
\textbf{Recommender} & \textbf{MIND} & \textbf{Micro.} & \textbf{Good.} & \textbf{CDs} & \textbf{H\&M} & \textbf{Overall} & \textbf{Latency} \\
\midrule
\rstt{}BERT$_\text{base}$ & 0.4963 & 0.4992 & 0.4958 & 0.5059 & 0.5204 & 0.5035 & 53.26ms \\
\rstt{}OPT$_\text{350M}$ & 0.5490 & 0.4773 & 0.5015 & 0.5093 & 0.4555 & 0.4985 & 332.34ms \\
\rstt{}OPT$_\text{1B}$ & 0.5338 & 0.5236 & 0.5042 & 0.4994 & 0.5650 & 0.5252 & 1.14s \\
\rstt{}Llama-1$_\text{7B}$ & 0.4583 & 0.4572 & 0.4994 & 0.4995 & 0.4035 & 0.4636 & 3.17s \\
\rstt{}Llama-2$_\text{7B}$ & 0.4945 & 0.4877 & 0.5273 & 0.5191 & 0.4519 & 0.4961 & 6.20s \\
\rstt{}Llama-3$_\text{8B}$ & 0.4904 & 0.5577 & 0.5191 & 0.5136 & 0.5454 & 0.5252 & 6.80s \\
\rstt{}Llama-3.1$_\text{8B}$ & 0.5002 & 0.5403 & 0.5271 & 0.5088 & 0.5462 & 0.5245 & 6.58s \\
\rstt{}Mistral$_\text{7B}$ & \underline{0.6300} & 0.6579 & \textbf{0.5718} & \underline{0.5230} & \underline{0.7166} & \underline{0.6199} & 7.68s \\
\rstt{}GLM-4$_\text{9B}$ & \textbf{0.6304} & \textbf{0.6647} & \underline{0.5671} & 0.5213 & \textbf{0.7319} & \textbf{0.6231} & 9.69s \\
\rstt{}Qwen-2$_\text{0.5B}$ & 0.4868 & 0.5717 & 0.5148 & 0.5043 & 0.6287 & 0.5413 & 543.73 \\
\rstt{}Qwen-2$_\text{1.5B}$ & 0.5411 & 0.6072 & 0.5264 & 0.5174 & 0.6615 & 0.5707 & 1.42s \\
\rstt{}Qwen-2$_\text{7B}$ & 0.5862 & \underline{0.6640} & 0.5494 & \textbf{0.5256} & 0.7124 & 0.6075 & 6.15s\\
\rstt{}DS-Qwen-2$_\text{7B}$ & 0.5127 & 0.5631 & 0.5165 & 0.5146 & 0.5994 & 0.5413 & 7.52s \\
\rstt{}Phi-2$_\text{3B}$ & 0.4851 & 0.5078 & 0.5049 & 0.4991 & 0.5447 & 0.5083 & 2.10s \\
\rstt{}GPT-3.5 & 0.5057 & 0.5110 & 0.5122 & 0.5046 & 0.5801 & 0.5227 & - \\
\midrule
\rstt{}RecGPT$_\text{7B}$ & 0.5078 & 0.4703 & 0.5083 & 0.5019 & 0.4875 & 0.4952 & 7.16s \\
\rstt{}P5$_\text{Beauty}$ & 0.4911 & 0.5017 & 0.5027 & 0.5447 & 0.4845 & 0.5049 & 74.11ms \\
\bottomrule
\end{tabular}
% }
\end{table}

==> Assets/Tables/llms.tex <==
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Large language and recommendation models benchmarked in our paper.}\label{tab:llm-list}

% \resizebox{\linewidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Model} & \textbf{Date} & \textbf{Size (M)} & \textbf{Institution}
% & \textbf{Source} 
\\
\midrule
\textbf{BERT$_\text{base}$} & 2018.10 & 110 & Google
% & \url{https://huggingface.co/google-bert/bert-base-uncased} 
\\
\textbf{OPT$_\text{base}$} & 2022.05 & 331 & Meta 
% & \url{https://huggingface.co/facebook/opt-350m} 
\\
\textbf{OPT$_\text{large}$} & 2022.05 & 1,316 & Meta 
% & \url{https://huggingface.co/facebook/opt-1.3b} 
\\
\textbf{GPT-3.5} & 2022.11 & - & OpenAI 
% & \url{https://platform.openai.com/docs/guides/text-generation} 
\\
\textbf{Llama-1$_\text{7B}$} & 2023.02 & 6,738 & Meta 
% & \url{https://huggingface.co/huggyllama/llama-7b} 
\\
% \textbf{E5-2} & 2023.05 & 109 & Microsoft 
% & \url{https://huggingface.co/intfloat/e5-base-v2} 
% \\
\textbf{Llama-2$_\text{7B}$} & 2023.06 & 6,738 & Meta 
% & \url{https://github.com/Llama-2-7b-hf} 
\\
\textbf{Phi-2} & 2023.10 & 2,780 & Microsoft 
% & \url{https://huggingface.co/microsoft/phi-2} 
\\
\textbf{GLM-4$_\text{9B}$} & 2024.01 & 9,400 & THU 
% & \url{https://huggingface.co/THUDM/glm-4-9b-chat} 
\\
\textbf{Mistral-2$_\text{7B}$} & 2024.02 & 7,248 & MistralAI 
% & \url{https://huggingface.co/mistralai/Mistral-7B-Instruct-v0.3} 
\\
\textbf{Llama-3$_\text{8B}$} & 2024.04 & 8,030 & Meta 
% & \url{https://huggingface.co/meta-llama/Meta-Llama-3-8B} 
\\
\textbf{Qwen-2$_\text{0.5B}$} & 2024.06 & 494 & Alibaba 
% & \url{https://huggingface.co/Qwen/Qwen2-0.5B-Instruct} 
\\
\textbf{Qwen-2$_\text{1.5B}$} & 2024.06 & 1,544 & Alibaba 
% & \url{https://huggingface.co/Qwen/Qwen2-1.5B-Instruct} 
\\
\textbf{Qwen-2$_\text{7B}$} & 2024.06 & 7,616 & Alibaba 
% & \url{https://huggingface.co/Qwen/Qwen2-7B-Instruct} 
\\
\textbf{Llama-3.1$_\text{8B}$} & 2024.06 & 8,030 & Meta 
% & \url{https://huggingface.co/meta-llama/Meta-Llama-3.1-8B} 
\\
\textbf{DeepSeek-Qwen-2$_\text{7B}$} & 2025.01 & 7,616 & DeepSeek 
% & \url{https://huggingface.co/deepseek-ai/DeepSeek-R1-Distill-Qwen-7B}
\\
\midrule
\textbf{P5} & 2022.03 & 223 & Rutgers. 
% & \url{https://huggingface.co/makitanikaze/P5} 
\\
\textbf{RecGPT$_\text{7B}$} & 2024.05 & 6,649 & VinAI 
% & \url{https://huggingface.co/vinai/RecGPT-7B} 
\\
\bottomrule
\end{tabular}
% }
\end{table}


==> Content/Acknowledgement.tex <==
\begin{ack}

\end{ack}

==> Content/RelatedWork.tex <==

\section{Related Work}

The evolution of using large language models directly as recommender systems (\llmasrs{}) can be divided into three stages, each closely related to the forms of item representation (\itemph{} in Figure~\ref{fig:scenarios}).

\noindent\textbf{Stage One: Early Zero-Shot \llmasrs{}.} In the initial stage, researchers explored whether general-purpose LLMs possess inherent recommendation abilities (shortly \textit{recabilities}) without any fine-tuning--a zero-shot setting. Experimental results indicated that while these methods~\citep{bm-lmasrs,reason-rec-1,reason-rec-2} did not outperform traditional recommendation models, they were more effective than purely random recommendations, demonstrating a limited but noteworthy ability for LLMs to make recommendations. Representative works in this stage include LMasRS~\citep{bm-lmasrs} based on BERT~\citep{llm-bert} and studies utilizing ChatGPT~\cite{llm-gpt35}. Since LLMs at this point could only process textual information, \stt{} was the sole form of item representation, serving as a bridge between LLMs and recommender systems across domains.

\noindent\textbf{Stage Two: Fine-Tuning LLMs for Recommendation.} In the second stage, researchers leveraged the deep reasoning abilities of LLMs by conducting supervised training on specific datasets to adapt them to recommendation scenarios. For example, Uni-CTR~\citep{unictr} and Recformer~\citep{recformer} continued to use semantic text as the medium for aligning recommender systems with LLMs, performing multi-scenario learning in pair-wise recommendation settings. Additionally, LLMs began to learn from non-textual signals during this phase. Models like P5~\citep{p5,openp5} and VIP5~\citep{vip5} used item \uid{} for multi-task training on Amazon datasets~\citep{ds-amazon}, covering tasks such as score prediction, next-item prediction, and review generation. Furthermore, LLaRA~\citep{llara} and LLM4IDRec~\citep{llm4idrec} fine-tuned LLMs in sequential recommendation scenarios, enabling them to handle user behavior sequences more effectively.

\noindent\textbf{Stage Three: Integration of Semantic Identifiers with LLMs.} In the most recent stage, researchers combined \sid{} with LLMs to enhance recommendation performance~\citep{llm-eager}. For instance, LC-Rec~\citep{lc-rec} extended the multi-task learning paradigm of P5 but replaced item representations with semantic identifiers, achieving breakthrough results. STORE~\citep{store} innovatively proposed a unified framework that integrates discrete semantic encoding with generative recommendation, further advancing the capabilities of LLM-based recommender systems in multiple recommendation scenarios.

% We have provided a more detailed classification of item representations and recommendation scenarios in Figure~\ref{fig:example}, highlighting representative works in each subarea. It is important to note that using LLMs to extract \sem{} is generally applied within traditional recommendation models, lacking further examples where LLMs themselves serve as recommender systems. Moreover, traditional sequential recommendation methods~\citep{sasrec,bert4rec} typically rely on next-item prediction to map to specific items, which is not suitable when using \stt{} as the item representation. Therefore, this paper focuses on evaluating and investigating the subareas highlighted with a blue background in Figure~\ref{fig:item-representation}.

